$K\to(\pi\pi)_{I=2}$ decays and twisted boundary conditions

We propose a new method to evaluate the Lellouch-L\"uscher factor which relates the $\Delta I=3/2$ $K\to\pi\pi$ matrix elements computed on a finite lattice to the physical (infinite-volume) decay amplitudes. The method relies on the use of partially twisted boundary conditions, which allow the s-wave $\pi\pi$ phase shift to be computed as an almost continuous function of the centre-of-mass relative momentum and hence for its derivative to be evaluated. We successfully demonstrate the feasibility of the technique in an exploratory computation.

==> two_pi_table.tex <==
\begin{tabular}{cccccc}
 Twist & Momentum & $E_{\pi\pi}$  & $E_{\pi,1}$ & $E_{\pi,2}$ & $\Delta E$ \\ \hline
$\frac{36}{36} \frac{\pi}{L} $ & 0  & 1.033(2) & 5.067e-1(3) & 5.067e-1(3) & 1.9e-2(2) \\ \hline 
$\frac{30}{36} \frac{\pi}{L} $ & $\frac{12}{36} \frac{\pi}{L}$  & 1.033(1) & 4.952e-1(3) & 5.197e-1(3) & 1.8e-2(1) \\ \hline 
$\frac{27}{36} \frac{\pi}{L} $ & $\frac{18}{36} \frac{\pi}{L}$  & 1.034(1) & 4.902e-1(3) & 5.269e-1(3) & 1.7e-2(1) \\ \hline 
$\frac{24}{36} \frac{\pi}{L} $ & $\frac{24}{36} \frac{\pi}{L}$  & 1.037(1) & 4.856e-1(3) & 5.344e-1(4) & 1.7e-2(1) \\ \hline 
$\frac{18}{36} \frac{\pi}{L} $ & $\frac{36}{36} \frac{\pi}{L}$  & 1.045(1) & 4.779e-1(3) & 5.505e-1(4) & 1.7e-2(1) \\ \hline 
$\frac{12}{36} \frac{\pi}{L} $ & $\frac{48}{36} \frac{\pi}{L}$  & 1.057(1) & 4.723e-1(3) & 5.678e-1(4) & 1.7e-2(1) \\ \hline 
$\frac{10}{36} \frac{\pi}{L} $ & $\frac{52}{36} \frac{\pi}{L}$  & 1.061(1) & 4.709e-1(3) & 5.738e-1(4) & 1.6e-2(1) \\ \hline 
$\frac{9}{36} \frac{\pi}{L} $ & $\frac{54}{36} \frac{\pi}{L}$  & 1.063(1) & 4.703e-1(3) & 5.768e-1(4) & 1.6e-2(1) \\ \hline 
$\frac{8}{36} \frac{\pi}{L} $ & $\frac{56}{36} \frac{\pi}{L}$  & 1.066(1) & 4.698e-1(3) & 5.799e-1(4) & 1.6e-2(1) \\ \hline 
$\frac{6}{36} \frac{\pi}{L} $ & $\frac{60}{36} \frac{\pi}{L}$  & 1.071(1) & 4.689e-1(3) & 5.862e-1(5) & 1.6e-2(1) \\ \hline 
$\frac{4}{36} \frac{\pi}{L} $ & $\frac{64}{36} \frac{\pi}{L}$  & 1.077(1) & 4.682e-1(3) & 5.925e-1(5) & 1.6e-2(1) \\ \hline 
$\frac{2}{36} \frac{\pi}{L} $ & $\frac{68}{36} \frac{\pi}{L}$  & 1.082(1) & 4.678e-1(3) & 5.990e-1(5) & 1.6e-2(1) \\ \hline 
0 & $\frac{72}{36} \frac{\pi}{L}$  & 1.089(1) & 4.676e-1(3) & 6.056e-1(5) & 1.5e-2(1) \\ \hline 
\end{tabular}

